GPTScan: Detecting Logic Vulnerabilities in Smart Contracts by Combining GPT with Program Analysis

Smart contracts are prone to various vulnerabilities, leading to substantial financial losses over time. Current analysis tools mainly target vulnerabilities with fixed control or data-flow patterns, such as re-entrancy and integer overflow. However, a recent study on Web3 security bugs revealed that about 80% of these bugs cannot be audited by existing tools due to the lack of domain-specific property description and checking. Given recent advances in Large Language Models (LLMs), it is worth exploring how Generative Pre-training Transformer (GPT) could aid in detecting logicc vulnerabilities. In this paper, we propose GPTScan, the first tool combining GPT with static analysis for smart contract logic vulnerability detection. Instead of relying solely on GPT to identify vulnerabilities, which can lead to high false positives and is limited by GPT's pre-trained knowledge, we utilize GPT as a versatile code understanding tool. By breaking down each logic vulnerability type into scenarios and properties, GPTScan matches candidate vulnerabilities with GPT. To enhance accuracy, GPTScan further instructs GPT to intelligently recognize key variables and statements, which are then validated by static confirmation. Evaluation on diverse datasets with around 400 contract projects and 3K Solidity files shows that GPTScan achieves high precision (over 90%) for token contracts and acceptable precision (57.14%) for large projects like Web3Bugs. It effectively detects ground-truth logic vulnerabilities with a recall of over 70%, including 9 new vulnerabilities missed by human auditors. GPTScan is fast and cost-effective, taking an average of 14.39 seconds and 0.01 USD to scan per thousand lines of Solidity code. Moreover, static confirmation helps GPTScan reduce two-thirds of false positives.

==> RQ6.tex <==
\subsection{RQ6: On the Dependency of GPT Models}

In this research question, we focus on the influence of different GPT models on the result of \name.
We used 3 different configurations of the GPT model:
\begin{itemize}
    \item 1. GPT-3.5, 0301 version, temperature of 1.
    \item 2. GPT-3.5, 0301 version, temperature of 0 (used in RQ1 to RQ5).
    \item 3. GPT-3.5, 0613 version, temperature of 0.
\end{itemize}
The \textit{temperature} is an hyperparameter of GPT model, which is used to control the randomness of the output. 
When the \textit{temperature} is 0, the output is deterministic, and when the \textit{temperature} is 1, the output is more random.
Version 0613 is a newer version of GPT-3.5, which is released on June 2023, and version 0301 is released on March 2023.
According to the research by Chen et al.~\cite{Chen_Zaharia_Zou_2023}, the behavior of GPT model become worse with the upgrade of the version.
The precision, recall, and accuracy of \name with different configurations on all 3 dataset are shown in Table~\ref{tab:logic_different_model}.
\begin{table}[htbp]
    \footnotesize
    \caption{Result of Different GPT Model}
    \label{tab:logic_different_model}
    \begin{tabular}{llrrr}
        \hline
        \textbf{Dataset} & \textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{Accuracy} \\ \hline
        \multirow{3}{*}{Top200} & 1 & - & - & 0.95 \\
        & 2 & - & - & 0.95 \\
        & 3 & - & - & \textbf{0.97} \\ \hline
        \multirow{3}{*}{Web3Bugs} & 1 & 0.42 & \textbf{0.83} & 0.79 \\
        & 2 & \textbf{0.57} & \textbf{0.83} & \textbf{0.83} \\
        & 3 & 0.32 & 0.54 & 0.75 \\ \hline
        \multirow{3}{*}{DefiHacks} & 1 & 0.62 & 0.62 & 0.72 \\
        & 2 & \textbf{0.91} & \textbf{0.71} & \textbf{0.85} \\
        & 3 & 0.75 & 0.69 & 0.80 \\ \hline
    \end{tabular}
\end{table}
In this table, we can find that the model configuration 2, which is GPT-3.5, 0301 version, temperature of 0, has the best performance on \textit{Web3Bugs} and \textit{DefiHacks}.
On \textit{Top200}, the model configuration 3, which is GPT-3.5, 0613 version, temperature of 0, has the best performance, which is 2\% better than the model configuration 2.
The higher temperature may help find some vulnerabilities that are difficult to be matched by scenarios and properties by GPT model, but it may also cause more false positive cases.
The result of this experiment shows that the performance of \name is influenced by the configurations of GPT model, and the newer version of GPT model may have a worse performance on detecting vulnerabilities.

\answerbox{
\textbf{Answer for RQ6: } The performance of \name is influenced by the version of GPT model. GPT-3.5 with 0301 version and temperature of 0 has the best performance on \textit{Web3Bugs} and \textit{DefiHacks}, and GPT-3.5 with 0613 version and temperature of 0 has the best performance on \textit{Top200}. The result showes that a higher temperature may help find some vulnerabilities that are difficult to be detected, but it may also harm the precision. The result also suggests that the newer version of GPT model may have a worse performance on detecting vulnerabilities.
}


==> learning.tex <==
\section{Learning Logic Properties}
\label{sec:learn}

